K3 surfaces and equations for Hilbert modular surfaces

We outline a method to compute rational models for the Hilbert modular surfaces Y_{-}(D), which are coarse moduli spaces for principally polarized abelian surfaces with real multiplication by the ring of integers in Q(sqrt{D}), via moduli spaces of elliptic K3 surfaces with a Shioda-Inose structure. In particular, we compute equations for all thirty fundamental discriminants D with 1 < D < 100, and analyze rational points and curves on these Hilbert modular surfaces, producing examples of genus-2 curves over Q whose Jacobians have real multiplication over Q.

==> jacobians <==

\\ p will be a quartic polynomial in x
\\ p(x) = a0*x^4 + 4*a1*x^3 + 6*a2*x^2 + 4*a3*x + a4

{
jac2(p) = 
local(a0,a1,a2,a3,a4,i,j);
a0 = polcoeff(p,4,x);
a1 = polcoeff(p,3,x)/4;
a2 = polcoeff(p,2,x)/6;
a3 = polcoeff(p,1,x)/4;
a4 = subst(p,x,0);

i = a0*a4 - 4*a1*a3 + 3*a2^2;
j = a0*a2*a4 + 2*a1*a2*a3 - a0*a3^2 - a4*a1^2 - a2^3;
return(x^3 - i/4*x - j/4);

}


\\ p will be a cubic polynomial in x and t
\\ p(x,t) = a*x^3 + b*t^3 + c + 3*a2*x^2*t+ 3*a3*x^2 + 3*b1*t^2*x + 3*b3*t^2 + 3*c1*x + 3*c2*t + 6*m*x*t
\\ returns coefficients for y^2 = 4*x^3 - g2*x - g3;


{
jac3(p) = 
local(a,b,c,a2,a3,b2,b3,c1,c2,m, S, T, g2, g3);
a = polcoeff(p,3,x);
b = polcoeff(p,3,t);
c = subst(subst(p,x,0),t,0);
a2 = polcoeff(polcoeff(p,2,x),1,t)/3;
a3 = subst(polcoeff(p,2,x),t,0)/3;
b1 = polcoeff(polcoeff(p,2,t),1,x)/3;
b3 = subst(polcoeff(p,2,t),x,0)/3;
c1 = subst(polcoeff(p,1,x),t,0)/3;
c2 = subst(polcoeff(p,1,t),x,0)/3;
m = polcoeff(polcoeff(p,1,x),1,t)/6;

S = a*b*c*m -  (b*c*a2*a3 + c*a*b1*b3 + a*b*c1*c2) - 
  m*(a*b3*c2 + b*c1*a3 + c*a2*b1) + (a*b1*c2^2 + a*c1*b3^2 + 
    b*a2*c1^2 + b*c2*a3^2 + c*b3*a2^2 + c*a3*b1^2) - m^4 + 
  2*m^2*(b1*c1 + c2*a2 + a3*b3) - 
  3*m*(a2*b3*c1 + a3*b1*c2) - (b1^2*c1^2 + c2^2*a2^2 + 
    a3^2*b3^2) + (c2*a2*a3*b3 + a3*b3*b1*c1 + b1*c1*c2*a2 );

T = 8*a3^3*b3^3 + 4*a3^3*b^2*c - 12*a2*a3^2*b*b3*c + 
  24*a3^2*b1^2*b3*c + 
    24*a2^2*a3*b3^2*c - 12*a*a3*b1*b3^2*c + 4*a^2*b3^3*c + 
  4*a2^3*b*c^2 + 
    a^2*b^2*c^2 - 6*a*a2*b*b1*c^2 - 3*a2^2*b1^2*c^2 + 4*a*b1^3*c^2 - 
    12*a3^2*b1*b3^2*c1 - 12*a*a3*b3^3*c1 - 6*a*a3*b^2*c*c1 + 
  18*a2*a3*b*b1*c*c1 - 
    12*a3*b1^3*c*c1 + 6*a*a2*b*b3*c*c1 + 6*a2^2*b1*b3*c*c1 - 
  12*a*b1^2*b3*c*c1 - 
    3*a3^2*b^2*c1^2 + 6*a2*a3*b*b3*c1^2 - 12*a3*b1^2*b3*c1^2 - 
    27*a2^2*b3^2*c1^2 + 24*a*b1*b3^2*c1^2 + 4*a*b^2*c1^3 - 
  12*a2*b*b1*c1^3 + 
    8*b1^3*c1^3 - 12*a3^3*b*b3*c2 - 12*a2*a3^2*b3^2*c2 - 
  12*a2^2*a3*b*c*c2 + 
    6*a*a3*b*b1*c*c2 + 6*a2*a3*b1^2*c*c2 - 12*a2^3*b3*c*c2 - 
  6*a^2*b*b3*c*c2 + 
    18*a*a2*b1*b3*c*c2 + 6*a3^2*b*b1*c1*c2 + 18*a*a3*b*b3*c1*c2 - 
    6*a2*a3*b1*b3*c1*c2 + 6*a*a2*b3^2*c1*c2 + 24*a2^2*b*c1^2*c2 - 
    12*a*b*b1*c1^2*c2 - 12*a2*b1^2*c1^2*c2 + 24*a2*a3^2*b*c2^2 - 
    27*a3^2*b1^2*c2^2 - 12*a2^2*a3*b3*c2^2 + 6*a*a3*b1*b3*c2^2 - 
    3*a^2*b3^2*c2^2 - 12*a*a2*b*c1*c2^2 - 12*a2^2*b1*c1*c2^2 + 
    24*a*b1^2*c1*c2^2 + 8*a2^3*c2^3 + 4*a^2*b*c2^3 - 12*a*a2*b1*c2^3 - 
    24*a3^2*b*b1*c*m + 12*a*a3*b*b3*c*m - 60*a2*a3*b1*b3*c*m - 
  24*a*a2*b3^2*c*m + 
    12*a3^2*b*b3*c1*m + 36*a2*a3*b3^2*c1*m - 24*a2^2*b*c*c1*m + 
    12*a*b*b1*c*c1*m + 12*a2*b1^2*c*c1*m + 12*a3*b*b1*c1^2*m - 
  24*a*b*b3*c1^2*m + 
    36*a2*b1*b3*c1^2*m + 36*a3^2*b1*b3*c2*m + 12*a*a3*b3^2*c2*m + 
    12*a*a2*b*c*c2*m + 12*a2^2*b1*c*c2*m - 24*a*b1^2*c*c2*m - 
    60*a2*a3*b*c1*c2*m + 36*a3*b1^2*c1*c2*m + 36*a2^2*b3*c1*c2*m - 
    60*a*b1*b3*c1*c2*m - 24*a*a3*b*c2^2*m + 36*a2*a3*b1*c2^2*m + 
    12*a*a2*b3*c2^2*m - 24*a3^2*b3^2*m^2 + 36*a2*a3*b*c*m^2 + 
  12*a3*b1^2*c*m^2 + 
    12*a2^2*b3*c*m^2 + 36*a*b1*b3*c*m^2 - 12*a3*b1*b3*c1*m^2 + 
  12*a*b3^2*c1*m^2 + 
    12*a2*b*c1^2*m^2 - 24*b1^2*c1^2*m^2 + 12*a3^2*b*c2*m^2 - 
  12*a2*a3*b3*c2*m^2 + 
    36*a*b*c1*c2*m^2 - 12*a2*b1*c1*c2*m^2 - 24*a2^2*c2^2*m^2 + 
  12*a*b1*c2^2*m^2 - 
    20*a*b*c*m^3 - 12*a2*b1*c*m^3 - 12*a3*b*c1*m^3 - 36*a2*b3*c1*m^3 - 
    36*a3*b1*c2*m^3 - 12*a*b3*c2*m^3 + 24*a3*b3*m^4 + 24*b1*c1*m^4 + 
    24*a2*c2*m^4 - 8*m^6;

g2 = -108*S;
g3 = 27*T;

return(x^3 - g2*x/4 - g3/4);
}



